Secrecy Transmission on Block Fading Channels: Theoretical Limits and Performance of Practical Codes

We consider a system where an agent (Alice) aims at transmitting a message to a second agent (Bob) over a set of parallel channels, while keeping it secret from a third agent (Eve) by using physical layer security techniques. We assume that Alice perfectly knows the set of channels with respect to Bob, but she has only a statistical knowledge of the channels with respect to Eve. We derive bounds on the achievable outage secrecy rates, by considering coding either within each channel or across all parallel channels. Transmit power is adapted to the channel conditions, with a constraint on the average power over the whole transmission. We also focus on the maximum cumulative outage secrecy rate that can be achieved. Moreover, in order to assess the performance in a real life scenario, we consider the use of practical error correcting codes. We extend the definitions of security gap and equivocation rate, previously applied to the single additive white Gaussian noise channel, to Rayleigh distributed parallel channels, on the basis of the error rate targets and the outage probability. Bounds on these metrics are also derived, taking into account the statistics of the parallel channels. Numerical results are provided, that confirm the feasibility of the considered physical layer security techniques.

==> CASfigure.tex <==
\begin{tikzpicture}
\def\radius{2mm} 
\tikzstyle{branch}=[fill,shape=circle,minimum size=3pt,inner sep=0pt]

	% Place nodes using a matrix
	\matrix (m1) [row sep=9mm, column sep=7mm]
	{
		%--------------------------------------------------------------------
		\node[dspnodeopen,dsp/label=above] (m00) {Alice};    &
		\node[dspfilter]  (m01) {\,ENC\, }; &
		\node[dspfilter]  (m02) {\,S/P\, }; &
		\node[dspmixer]   (m03) {};    &		
		\node[dspnodefull](m04) {};          &
		\node[coordinate](m05) {};          &				
		\node[dspmixer]   (m06) {};    &
		\node[dspadder]   (m07) {};    &
		\node[dspfilter]  (m08) {\,P/S\,}; &		
		\node[dspfilter]  (m09) {\,DEC\, }; &		
		\node[dspnodeopen,dsp/label=above] (m010) {Bob};    
\\
		%--------------------------------------------------------------------
		\node[coordinate] (m10) {};    &
		\node[coordinate] (m11) {};    &		
		\node[coordinate] (m12) {}; &
		\node[dspmixer]   (m13) {};    &		
		\node[coordinate] (m14) {};          &
		\node[coordinate] (m15) {};          &		
		\node[dspmixer, dsp/label=below]   (m16) {};    &
		\node[dspadder]   (m17) {};    &
		\node[coordinate]  (m18) {}; &			
		\node[coordinate] (m19) {};    
\\
		%--------------------------------------------------------------------
		\node[coordinate] (p00) {};    &
		&
		&
		&		
		\node[coordinate](p04) {};          &
		\node[coordinate](p05) {};          &				
		\node[dspmixer]   (p06) {};    &
		\node[dspadder]   (p07) {};    &
		\node[dspfilter]  (p08) {\,P/S\,}; &		
		\node[dspfilter]  (p09) {\,DEC\, }; &		
		\node[dspnodeopen,dsp/label=above] (p010) {Eve};    
\\
		%--------------------------------------------------------------------
		&
		&		
		&
		&		
		&
		\node[coordinate] (p15) {};          &		
		\node[dspmixer, dsp/label=below]   (p16) {};    &
		\node[dspadder]   (p17) {};    &
		\node[coordinate]  (p18) {}; &			
		\node[coordinate] (p19) {};  \\
	};

	% Draw connections

	\foreach \i [evaluate = \i as \j using int(\i),
	             evaluate = \i as \k using int(\i+1),] in {0,1,2,6,7}
	{
		\begin{scope}[start chain]
			\chainin (m0\i);
			\chainin (m0\k) [join=by dspconn];
		\end{scope}
	}
		\begin{scope}[start chain]
			\chainin (m09);
			\chainin (m010) [join=by dspconn];
		\end{scope}
		\begin{scope}[start chain]
			\chainin (m03);
			\chainin (m06) [join=by dspconn];
		\end{scope}


   \draw[dspline] (m02.-20)+(.4, 0) node {}{} -- (m02.-20)+(.4, 0);           
   \draw[dspconn] (m02.-20)+(.4, 0) node[above] {}{} |- (m13.west);        


\path [draw, dspconn] (m08) -- node [above] {} 
        (m09) ;
\path [draw, dspline] (m17.0)+(.4,0) -- 	(m17.0)+(.4,0) ;
   \draw[dspconn] (m17.east)+(.4,0) node {}{} |- (m08.200);           
          

        
	\foreach \i [evaluate = \i as \j using int(\i),
	             evaluate = \i as \k using int(\i+1),] in {6}
	{

		\begin{scope}[start chain]
			\chainin (m1\i);
			\chainin (m1\k) [join=by dspconn];
		\end{scope}

	}
		\begin{scope}[start chain]
			\chainin (m13);
			\chainin (m16) [join=by dspconn];
		\end{scope}

	\foreach \i [evaluate = \i as \j using int(\i),
	             evaluate = \i as \k using int(\i+1),] in {6,7}
	{
		\begin{scope}[start chain]
			\chainin (p0\i);
			\chainin (p0\k) [join=by dspconn];
		\end{scope}
	}
		\begin{scope}[start chain]
			\chainin (p09);
			\chainin (p010) [join=by dspconn];
		\end{scope}
%		\begin{scope}[start chain]
%			\chainin (p04);
%			\chainin (p06) [join=by dspconn];
%		\end{scope}

\path [draw, dspconn] (p08) -- 	(p09) ;	
\path [draw, dspline] (p17.0)+(.4,0) -- 	(p17.0)+(.4,0) ;	
\draw[dspconn] (p17.east)+(.4,0) node {}{} |- (p08.200);      
                      
	\foreach \i [evaluate = \i as \j using int(\i),
	             evaluate = \i as \k using int(\i+1),] in {6}
	{

		\begin{scope}[start chain]
			\chainin (p1\i);
			\chainin (p1\k) [join=by dspconn];
		\end{scope}

	}



\node[draw=white, below of=m03] (E) {$\sqrt{P_1}$};
\node[draw=white, below of=m13] (E2) {$\sqrt{P_K}$};
\node[draw=white, below of=m06] (A) {$h_1$};
\node[draw=white, below of=m16] (B) {$h_K$};
\node[draw=white, below of=m07] (C) {noise};
\node[draw=white, below of=m17] (D) {noise};
\draw[dspconn] (E) -- (m03);
\draw[dspconn] (E2) -- (m13);
\draw[dspconn] (A) -- (m06);
\draw[dspconn] (B) -- (m16);
\draw[dspconn] (C) -- (m07);
\draw[dspconn] (D) -- (m17);

\node[draw=white, below of=p06] (pA) {$g_1$};
\node[draw=white, below of=p16] (pB) {$g_K$};
\node[draw=white, below of=p07] (pC) {noise};
\node[draw=white, below of=p17] (pD) {noise};


\node[draw=white, below of=m05, rotate=90] (punti1) {...};

\draw[dspconn] (pA) -- (p06);
\draw[dspconn] (pB) -- (p16);
\draw[dspconn] (pC) -- (p07);
\draw[dspconn] (pD) -- (p17);

    \tikzstyle{s}=[shift={(0mm,\radius)}]
   \draw[dspconn] (m04) node[branch] {}{ % draw branch junction
                [shift only] -- ([s]m14 -| m04) arc(90:-90:\radius)
        } |- (p06);
   \draw[dspconn] (m15) node[branch] {}{ % draw branch junction
                [shift only] -- ([s]p05 -| m15) arc(90:-90:\radius)
        } |- (p16);
        
\end{tikzpicture}

==> CPSfigure.tex <==
\begin{tikzpicture}
\def\radius{2mm} 
\tikzstyle{branch}=[fill,shape=circle,minimum size=3pt,inner sep=0pt]

	% Place nodes using a matrix
	\matrix (m1) [row sep=9mm, column sep=7mm]
	{
		%--------------------------------------------------------------------
		\node[dspnodeopen,dsp/label=above] (m00) {Alice};    &
		\node[dspfilter]  (m01) {\,S/P\, }; &
		\node[dspfilter]  (m02) {\,ENC\, }; &
		\node[dspmixer]   (m03) {};    &		
		\node[dspnodefull](m04) {};          &
		\node[coordinate](m05) {};          &				
		\node[dspmixer]   (m06) {};    &
		\node[dspadder]   (m07) {};    &
		\node[dspfilter]  (m08) {\,DEC\,}; &		
		\node[dspfilter]  (m09) {\,P/S\, }; &		
		\node[dspnodeopen,dsp/label=above] (m010) {Bob};    
\\
		%--------------------------------------------------------------------
		\node[coordinate] (m10) {};    &
		\node[coordinate] (m11) {};    &		
		\node[dspfilter]  (m12) {\,ENC\, }; &
		\node[dspmixer]   (m13) {};    &		
		\node[coordinate] (m14) {};          &
		\node[coordinate] (m15) {};          &		
		\node[dspmixer, dsp/label=below]   (m16) {};    &
		\node[dspadder]   (m17) {};    &
		\node[dspfilter]  (m18) {\,DEC\,}; &			
		\node[coordinate] (m19) {};    
\\
		%--------------------------------------------------------------------
		\node[coordinate] (p00) {};    &
		&
		&
		&		
		\node[coordinate](p04) {};          &
		\node[coordinate](p05) {};          &				
		\node[dspmixer]   (p06) {};    &
		\node[dspadder]   (p07) {};    &
		\node[dspfilter]  (p08) {\,DEC\,}; &		
		\node[dspfilter]  (p09) {\,P/S\, }; &		
		\node[dspnodeopen,dsp/label=above] (p010) {Eve};    
\\
		%--------------------------------------------------------------------
		&
		&		
		&
		&		
		&
		\node[coordinate] (p15) {};          &		
		\node[dspmixer, dsp/label=below]   (p16) {};    &
		\node[dspadder]   (p17) {};    &
		\node[dspfilter]  (p18) {\,DEC\,}; &			
		\node[coordinate] (p19) {};    
		\\
	};

	% Draw connections

	\foreach \i [evaluate = \i as \j using int(\i),
	             evaluate = \i as \k using int(\i+1),] in {0,2,6,7}
	{
		\begin{scope}[start chain]
			\chainin (m0\i);
			\chainin (m0\k) [join=by dspconn];
		\end{scope}
	}
		\begin{scope}[start chain]
			\chainin (m09);
			\chainin (m010) [join=by dspconn];
		\end{scope}
		\begin{scope}[start chain]
			\chainin (m03);
			\chainin (m06) [join=by dspconn];
		\end{scope}

   \draw[dspconn] (m01.20) node[above] {}{} |- (m02.160);
   \draw[dspline] (m01.-20)+(.4, 0) node {}{} -- (m01.-20)+(.4, 0);           
   \draw[dspconn] (m01.-20)+(.4, 0) node[above] {}{} |- (m12.west);        


\path [draw, dspconn] (m08.20) -- node [above] {} 
        (m09.160) ;
\path [draw, dspline] (m18.0)+(.4,0) -- 	(m18.0)+(.4,0) ;
   \draw[dspconn] (m18.east)+(.4,0) node {}{} |- (m09.200);           
          

        
	\foreach \i [evaluate = \i as \j using int(\i),
	             evaluate = \i as \k using int(\i+1),] in {2,6,7}
	{

		\begin{scope}[start chain]
			\chainin (m1\i);
			\chainin (m1\k) [join=by dspconn];
		\end{scope}

	}
		\begin{scope}[start chain]
			\chainin (m13);
			\chainin (m16) [join=by dspconn];
		\end{scope}

	\foreach \i [evaluate = \i as \j using int(\i),
	             evaluate = \i as \k using int(\i+1),] in {6,7}
	{
		\begin{scope}[start chain]
			\chainin (p0\i);
			\chainin (p0\k) [join=by dspconn];
		\end{scope}
	}
		\begin{scope}[start chain]
			\chainin (p09);
			\chainin (p010) [join=by dspconn];
		\end{scope}
%		\begin{scope}[start chain]
%			\chainin (p04);
%			\chainin (p06) [join=by dspconn];
%		\end{scope}

\path [draw, dspconn] (p08.20) -- 	(p09.160) ;	
\path [draw, dspline] (p18.0)+(.4,0) -- 	(p18.0)+(.4,0) ;	
\draw[dspconn] (p18.east)+(.4,0) node {}{} |- (p09.200);      
                      
	\foreach \i [evaluate = \i as \j using int(\i),
	             evaluate = \i as \k using int(\i+1),] in {6,7}
	{

		\begin{scope}[start chain]
			\chainin (p1\i);
			\chainin (p1\k) [join=by dspconn];
		\end{scope}

	}



\node[draw=white, below of=m03] (E) {$\sqrt{P_1}$};
\node[draw=white, below of=m13] (E2) {$\sqrt{P_K}$};
\node[draw=white, below of=m06] (A) {$h_1$};
\node[draw=white, below of=m16] (B) {$h_K$};
\node[draw=white, below of=m07] (C) {noise};
\node[draw=white, below of=m17] (D) {noise};
\draw[dspconn] (E) -- (m03);
\draw[dspconn] (E2) -- (m13);
\draw[dspconn] (A) -- (m06);
\draw[dspconn] (B) -- (m16);
\draw[dspconn] (C) -- (m07);
\draw[dspconn] (D) -- (m17);

\node[draw=white, below of=p06] (pA) {$g_1$};
\node[draw=white, below of=p16] (pB) {$g_K$};
\node[draw=white, below of=p07] (pC) {noise};
\node[draw=white, below of=p17] (pD) {noise};
\node[draw=white, below of=m02, rotate=90] (punti) {...};
\node[draw=white, below of=m08, rotate=90] (punti1) {...};
\node[draw=white, below of=m05, rotate=90] (punti1) {...};
\node[draw=white, below of=p08, rotate=90] (punti2) {...};
\draw[dspconn] (pA) -- (p06);
\draw[dspconn] (pB) -- (p16);
\draw[dspconn] (pC) -- (p07);
\draw[dspconn] (pD) -- (p17);

    \tikzstyle{s}=[shift={(0mm,\radius)}]
   \draw[dspconn] (m04) node[branch] {}{ % draw branch junction
                [shift only] -- ([s]m14 -| m04) arc(90:-90:\radius)
        } |- (p06);
   \draw[dspconn] (m15) node[branch] {}{ % draw branch junction
                [shift only] -- ([s]p05 -| m15) arc(90:-90:\radius)
        } |- (p16);
        
\end{tikzpicture}


==> tikzlibrarydsp.code.tex <==
% -------------------------------------------------------------------------
% This library for block diagrams and signal flow graphs was inspired by
% the library "signalflow" of Dr. Karlheinz Ochs, Ruhr-University of Bochum,
% Germany. Furthermore, some ideas were taken from the library "circuitikz"
% of Massimo A. Redaelli and from the PGF library itself.
%
% Copyright 2012 by Matthias Hotz
%
% This work is licensed under the Creative Commons Attribution 2.5 Generic
% License. To view a copy of this license, visit
%          http://creativecommons.org/licenses/by/2.5/
% or send a letter to Creative Commons, 444 Castro Street, Suite 900,
% Mountain View, California, 94041, USA.
% -------------------------------------------------------------------------

\usetikzlibrary{arrows, calc, positioning, decorations.markings}

% -------------------------------------------------------------------------
% Parameters for the library

\newcommand{\dsplinewidth}{0.25mm}           % Line width for connections
\newcommand{\dspblocklinewidth}{0.3mm}       % Line width for blocks
\newcommand{\dspoperatordiameter}{4mm}       % Diameter for adder, multiplier, mixer
\newcommand{\dspoperatorlabelspacing}{2mm}   % Distance from symbol to label for adder, multiplier, mixer
\newcommand{\dspnoderadius}{1mm}             % Filled and empty node
\newcommand{\dspsquareblocksize}{8mm}        % Size for square blocks, e.g. for delay elements, decimator, expander
\newcommand{\dspfilterwidth}{8mm}           % Width of a filter block

% -------------------------------------------------------------------------
% Define new arrow heads

\pgfarrowsdeclare{dsparrow}{dsparrow}
{
	\arrowsize=0.25pt
	\advance\arrowsize by .5\pgflinewidth
	\pgfarrowsleftextend{-4\arrowsize}
	\pgfarrowsrightextend{4\arrowsize}
}
{
	\arrowsize=0.25pt
	\advance\arrowsize by .5\pgflinewidth
	\pgfsetdash{}{0pt} % Solid line (do not dash)
	\pgfsetmiterjoin	 % Fixed miter join of line
	\pgfsetbuttcap		 % Fixed butt cap of line
	\pgfpathmoveto{\pgfpoint{-4\arrowsize}{2.5\arrowsize}}
	\pgfpathlineto{\pgfpoint{4\arrowsize}{0pt}}
	\pgfpathlineto{\pgfpoint{-4\arrowsize}{-2.5\arrowsize}}
	\pgfpathclose
	\pgfusepathqfill
}

\pgfarrowsdeclare{dsparrowmid}{dsparrowmid}
{
	\arrowsize=0.25pt
	\advance\arrowsize by .5\pgflinewidth
	\pgfarrowsleftextend{-4\arrowsize}
	\pgfarrowsrightextend{4\arrowsize}
}
{
	\arrowsize=0.25pt
	\advance\arrowsize by .5\pgflinewidth
	\pgfsetdash{}{0pt}
	\pgfsetmiterjoin
	\pgfsetbuttcap
	\pgfpathmoveto{\pgfpoint{0}{2.5\arrowsize}}
	\pgfpathlineto{\pgfpoint{8\arrowsize}{0pt}}
	\pgfpathlineto{\pgfpoint{0}{-2.5\arrowsize}}
	\pgfpathclose
	\pgfusepathqfill
}

% -------------------------------------------------------------------------
% Define new node shapes

\makeatletter

\pgfkeys{/tikz/dsp/label/.initial=above}

% Generic shape generator for operators, i.e. nodes with a circular
% shape with an additional customizable drawing and a text label
\long\def\dspdeclareoperator#1#2{
	\pgfdeclareshape{#1}
	{
		% Saved anchors, macros and dimensions
		\savedanchor\centerpoint{\pgfpointorigin}
		\savedmacro\label{\def\label{\pgfkeysvalueof{/tikz/dsp/label}}}
	  \saveddimen\radius
	  {
		  \pgfmathsetlength\pgf@xa{\pgfshapeminwidth}
		  \pgfmathsetlength\pgf@ya{\pgfshapeminheight}
	    \ifdim\pgf@xa>\pgf@ya
	      \pgf@x=.5\pgf@xa
	    \else
	      \pgf@x=.5\pgf@ya
	    \fi
	  }
	  
	  % Inherit all anchors from the 'circle'-shape:
	  \inheritanchor[from={circle}]{center}
	  \inheritanchor[from={circle}]{mid}
	  \inheritanchor[from={circle}]{base}
	  \inheritanchor[from={circle}]{north}
	  \inheritanchor[from={circle}]{south}
	  \inheritanchor[from={circle}]{west}
	  \inheritanchor[from={circle}]{east}
	  \inheritanchor[from={circle}]{mid west}
	  \inheritanchor[from={circle}]{mid east}
	  \inheritanchor[from={circle}]{base west}
	  \inheritanchor[from={circle}]{base east}
	  \inheritanchor[from={circle}]{north west}
	  \inheritanchor[from={circle}]{south west}
	  \inheritanchor[from={circle}]{north east}
	  \inheritanchor[from={circle}]{south east}
	  \inheritanchorborder[from={circle}]
	  
	  % Draw circle and embed additional code
	  \backgroundpath
	  {
	    % Draw circle
	    \pgfpathcircle{\centerpoint}{\radius}
	    
	    % Embed additional code
	    % (Note that this code must call e.g. \pgfusepathqstroke
	    #2
	  }
	
		% Define anchor parametrized by the PGF key /tikz/dsp/label
	  \anchor{text}
	  {
			\centerpoint
			%
	    \def\templabelabove{above}
	    \def\templabelbelow{below}
	    \def\templabelleft{left}
	    \def\templabelright{right}
	    \pgfutil@tempdima=\dspoperatorlabelspacing
	    %
	    \ifx\label\templabelabove
				\advance\pgf@x by -0.5\wd\pgfnodeparttextbox
				\advance\pgf@y by \radius
				\advance\pgf@y by \pgfutil@tempdima
	    \fi
	    %
	    \ifx\label\templabelbelow
				\advance\pgf@x by -0.5\wd\pgfnodeparttextbox
				\advance\pgf@y by -\radius
				\advance\pgf@y by -\pgfutil@tempdima
				\advance\pgf@y by -\ht\pgfnodeparttextbox
	    \fi
	    %
	    \ifx\label\templabelleft
				\advance\pgf@x by -\radius
				\advance\pgf@x by -\pgfutil@tempdima
				\advance\pgf@x by -\wd\pgfnodeparttextbox
				\advance\pgf@y by -0.5\ht\pgfnodeparttextbox
				\advance\pgf@y by +0.5\dp\pgfnodeparttextbox
	    \fi
	    %
	    \ifx\label\templabelright
				\advance\pgf@x by \radius
				\advance\pgf@x by \pgfutil@tempdima
				\advance\pgf@y by -0.5\ht\pgfnodeparttextbox
				\advance\pgf@y by +0.5\dp\pgfnodeparttextbox
	    \fi
	  }
	}
}

\dspdeclareoperator{dspshapecircle}{\pgfusepathqstroke}

\dspdeclareoperator{dspshapecirclefull}{\pgfusepathqfillstroke}

\dspdeclareoperator{dspshapeadder}{
	% Coordinate offset for the plus
	\pgfutil@tempdima=\radius
	\pgfutil@tempdima=0.55\pgfutil@tempdima
	
	% Draw plus
	\pgfmoveto{\pgfpointadd{\centerpoint}{\pgfpoint{0pt}{-\pgfutil@tempdima}}}
	\pgflineto{\pgfpointadd{\centerpoint}{\pgfpoint{0pt}{ \pgfutil@tempdima}}}
	
	\pgfmoveto{\pgfpointadd{\centerpoint}{\pgfpoint{-\pgfutil@tempdima}{0pt}}}
	\pgflineto{\pgfpointadd{\centerpoint}{\pgfpoint{ \pgfutil@tempdima}{0pt}}}
	
	\pgfusepathqstroke
}

\dspdeclareoperator{dspshapemixer}{
	% Coordinate offset for the cross
	\pgfutil@tempdima=\radius
	\pgfutil@tempdima=0.707106781\pgfutil@tempdima
	
	% Draw cross
	\pgfmoveto{\pgfpointadd{\centerpoint}{\pgfpoint{-\pgfutil@tempdima}{-\pgfutil@tempdima}}}
	\pgflineto{\pgfpointadd{\centerpoint}{\pgfpoint{ \pgfutil@tempdima}{ \pgfutil@tempdima}}}
	
	\pgfmoveto{\pgfpointadd{\centerpoint}{\pgfpoint{-\pgfutil@tempdima}{ \pgfutil@tempdima}}}
	\pgflineto{\pgfpointadd{\centerpoint}{\pgfpoint{ \pgfutil@tempdima}{-\pgfutil@tempdima}}}
	
	\pgfusepathqstroke
}

\makeatother

% -------------------------------------------------------------------------
% Define node styles

\tikzset{dspadder/.style={shape=dspshapeadder,line cap=rect,line join=rect,
	line width=\dspblocklinewidth,minimum size=\dspoperatordiameter}}
\tikzset{dspmultiplier/.style={shape=dspshapecircle,line cap=rect,line join=rect,
	line width=\dspblocklinewidth,minimum size=\dspoperatordiameter}}
\tikzset{dspmixer/.style={shape=dspshapemixer,line cap=rect,line join=rect,
	line width=\dspblocklinewidth,minimum size=\dspoperatordiameter}}

\tikzset{dspnodeopen/.style={shape=dspshapecircle,line width=\dsplinewidth,minimum size=\dspnoderadius}}
\tikzset{dspnodefull/.style={shape=dspshapecirclefull,line width=\dsplinewidth,fill,minimum size=\dspnoderadius}}

% The fixed specification of text height and text depth is the somewhat
% unaesthetic workaround to align the text in different node at the same
% baseline. See the PGF/TikZ manual, ch. 5.1.
\tikzset{dspsquare/.style={shape=rectangle,draw,align=center,text depth=0.3em,text height=1em,inner sep=0pt,
	line cap=round,line join=round,line width=\dsplinewidth,minimum size=\dspsquareblocksize}}
\tikzset{dspfilter/.style={shape=rectangle,draw,align=center,text depth=0.3em,text height=1em,inner sep=0pt,
	line cap=round,line join=round,line width=\dsplinewidth,minimum height=\dspsquareblocksize,minimum width=\dspfilterwidth}}

% -------------------------------------------------------------------------
% Define "signal flow" lines

\tikzset{dspline/.style={line width=\dsplinewidth},line cap=round,line join=round}
\tikzset{dspconn/.style={->,>=dsparrow,line width=\dsplinewidth},line cap=round,line join=round}%line cap=rect,line join=miter}
\tikzset{dspflow/.style={line width=\dsplinewidth,line cap=round,line join=round,
  decoration={markings,mark=at position 0.5 with {\arrow{dsparrowmid}}},postaction={decorate}}}

% -------------------------------------------------------------------------
% Define various utility macros

\newcommand{\downsamplertext}[1]{\raisebox{0.1em}{$\big\downarrow$}#1}
\newcommand{\upsamplertext}[1]{\raisebox{0.1em}{$\big\uparrow$}#1}

